Datum-Wise Classification: A Sequential Approach to Sparsity

We propose a novel classification technique whose aim is to select an appropriate representation for each datapoint, in contrast to the usual approach of selecting a representation encompassing the whole dataset. This datum-wise representation is found by using a sparsity inducing empirical risk, which is a relaxation of the standard L 0 regularized risk. The classification problem is modeled as a sequential decision process that sequentially chooses, for each datapoint, which features to use before classifying. Datum-Wise Classification extends naturally to multi-class tasks, and we describe a specific case where our inference has equivalent complexity to a traditional linear classifier, while still using a variable number of features. We compare our classifier to classical L 1 regularized linear models (L 1-SVM and LARS) on a set of common binary and multi-class datasets and show that for an equal average number of features used we can get improved performance using our method.

==> sections/datawise.tex <==

We consider the problem of supervised multiclass classification\footnote{Note that this includes the binary supervised classification problem.} where the goal is to learn a classification function $f_\theta : \mathcal{X} \rightarrow \mathcal{Y}$ that associates one category $y \in \mathcal{Y}$ to a vector $x \in \mathcal{X}$ where $\mathcal{X} = \mathbb{R}^n$, $n$ being the dimension of the input vector.  Let $\theta$ be the vector of parameters to be learned from a training set composed of input/output pairs $\mathcal{T} = \{(x_i,y_i)\}_{i \in [1,N]}$.  These parameters are commonly found by minimizing the empirical risk defined by:
\begin{equation}
\theta^*=\argmin_\theta \frac{1}{T}\sum\limits_{i=1}^{T} \Delta(f_\theta(x_i),y_i),
\end{equation}
where $\Delta$ is the loss associated to a prediction error.\\

This empirical risk minimization problem does not consider any \textit{prior assumption} or constraint concerning the shape of the solution, and can result in overfitting models. Moreover, when facing a very large number of features, obtained solutions usually need to perform computations on all the features for classifying any input, resulting in models that are not very fast. We propose a different risk minimization problem where we add a regularization term that encourages the obtained classifier to classify using \textbf{on average} as few features as possible. In comparison to classical $L_0$ or $L_1$ regularized approaches, where the goal is to constraint the number of features used at the dataset level, our approach performs sparsity at the datum level.  Thus, our classifier may use different feature-sets depending on the datum being classified. This results in a \textbf{datum-wise sparse classifier} that uses few features for classifying easy inputs, and more features for classifying difficult or ambigous inputs.

We propose a classification problem where the classifier is a function that, in addition to predicting a label $y$ given an input $x$, also provides information about which features have been used for classification. Let us define $\mathcal{Z} = [0;1]^m$. We define a \textbf{data-wise classification function} $f$ of parameters $\theta$ as:
\begin{equation}
 g_\theta : \begin{cases}
 						 \mathcal{X} \rightarrow \mathcal{Y} \times \mathcal{Z} \\
 						 f_\theta(x) = (y,z)
 						\end{cases}
\label{eq:loss}
\end{equation}
where $y$ is the predicted output and $z$ is a $m$-dimensional vector $z=(z^1,...,z^m)$, where $z^i=1$ means that features $i$ has been used for computing $y$. By convention, we will denote the predicted label as $y_\theta(x)$ and the corresponding $z$ vector as $z_\theta(x)$. When $z_\theta^i(x)=1$, feature $i$ as been used for classifying $x$ into category $y_\theta(x)$.

This definition of a datum-wise classifier has two main advantages: As explained hereafter, by explaining the classification process $z_\theta(x)$ it allows us to add constraint on the features used for classification resulting in the data-wise sparsity defined below. While this is not the main focus of our article, it allows one to obtain qualitative reasons explaining how the classification decision has been made - see part XX for a qualitative study of our approach.

Note that the way we defined datum-wise classification is an extension on the usual definition of a classifier.  Additionally, classical sparse classifier optimizing an $L_1$-regularized loss function can be described by a special case of our model where all the inputs of the classifier must have the same $z_\theta$, i.e. $\forall x = x', z_\theta(x) = z_\theta(x')$.
Note that our definition of a datum-wise classifier is an extension of the usual classifier definition.  Classical sparse classifiers that result from a $L_1$ regularized loss optimization corresponds to a special case of our model where same for all the input to classify i.e $\forall x = x', z_\theta(x) = z_\theta(x')$.

The data-wise sparsity is obtained by adding a regularization term on the empirical loss defined in equation \ref{eq:loss} that limit the average number of features used for classifying:
\begin{equation}
\theta^*=\argmin_\theta \frac{1}{T}\sum\limits_{i=1}^{T} \Delta(y_\theta(x_i),y_i) + \lambda \frac{1}{N} \sum\limits_{i=1}^{N} L_0(z_\theta(x_i))
\label{eq:datawiseloss}
\end{equation}
The regularization term $L_0(z_\theta(x_i))$ corresponds to the number of features selected for classifying $x_i$ - the number of $1$ in $z_\theta(x)$. In the general case, the minimization of this new risk results in a classifier that \textit{on average} select only a few features for classifying - but the features used can be different w.r.t to the input to classify.

Note that, when using classical classifiers - linear models for example - where  $\forall x = x', z_\theta(x) = z_\theta(x') = z_\theta$, this regularized loss is equivalent to the $L_0$ classical regularization defined in the literature [XX],[XX]. \\

The optimization of the loss defined in equation \ref{eq:datawiseloss} is a combinatorial problem which cannot be solved easily. We propose in the next section of the paper an original way to deal with such a problem based on sequential decision processes.

\section{Data-wise Sparse Sequential Classification}

\subsection{General Idea}

We consider a sequential model where an agent have to classify an input $x \in \mathbb{R}^n$. At the begining, the agent has no information about $x$. Then at each step, the agent can choose to acquire a particular features of $x$ or to classify $x$. the choice of classify $x$ in category $y$ ends the sequential process. XXfigureXX

\subsection{Sparse Sequential Classifier}

Let us denote $t$ the classification step - $t=0$ is the initial step and $T_{\theta}(x)$ the final step before choosing a category. Classifying an example $x$ corresponds to build a trajectory $(z^{0}_\theta(x),...,z^{T_{\theta}(x)}_\theta, y_\theta(x))$ where $z^t_\theta(x)$ corresponds to the subset of features selectionned by the agent at time $t$. The final classification action $z_\theta(x)$ is then only based on the subset of features $z^{T_{\theta}(x)}_\theta(x)$. Note that, $z^{0}_\theta(x)=0$ corresponds to the empty set of features and that switching from $z^{t}_\theta(x)$ to $z^{t+1}_\theta(x)$ is made by adding in $z^{t}_\theta(x)$ one feature that is not already in this set. The size $|z^{t}_\theta(x)|$ of $z^{t}_\theta(x)$ is thus equal to $t$.

The modelization of such a process can be made by using a \textit{Deterministic Markov Decision Process} which is a formalism usually used for describing sequential processes and reinforcement learning problems and techniques. As we consider here a very particular and simple case of MDP, we propose a lighter formalism which will refer to the usual MDP terminology. Considering the loss defined in equation XX, we define an optimal policy as a value of the parameters $\theta$ denoted $\theta^*$ such as :
\begin{equation}
\theta^*=\argmin_\theta \frac{1}{N}\sum\limits_{i=1}^{N} \Delta(y_{\theta}(x_i),y_i) + \lambda \frac{1}{N} \sum\limits_{i=1}^{N} |z^{T_\theta(x)}_\theta(x_i)|
\end{equation}

This risk can be rewritten as a average of indiviudal risks such as:
\begin{equation}
\begin{aligned}
	\theta^* & =\argmin_\theta \frac{1}{N}\sum\limits_{i=1}^{N} \left( \Delta(y_{\theta}(x_i),y_i) + \lambda |z^{T_\theta(x)}_\theta(x_i)| \right) \\
	 &=\argmax_\theta \frac{1}{N} \sum\limits_{i=1}^{N} R_\theta(x)
\end{aligned}
\end{equation}
where $R_\theta(x) = -\Delta(y_{\theta}(x_i),y_i) + \lambda |z^{T_\theta(x)}_\theta(x_i)|$ corresponds to the reward obtained by the classification agent $\theta$ at the end of the process of classifying $x$. The minimization of the classification loss is thus equivalent to finding an optimal policy $\theta^*$ that maximizes  a reward function $R(x)$ over a training set and very close to Reinforcement Learning problems with the difference of the existence of a training set and a testing set where not reward is available. This kind of approach has already been studied in different contexts like graph mining [PETERS] or structured output classification [MAES]. At each step $t$ the agent can choose between two types of actions in the set $\mathcal{A}$:
\begin{itemize}
\item A \textit{feature selection} action that consists in adding one new feature to the set of already chosen ones. Such an action results in transiting from $z^t_\theta(x)$ to $z^{t+1}_\theta(x)$. The agent can choose any of the remaining features resulting in $n-t$ possible actions - see section XX for a discussion about the complexity of such an approach
\item A \textit{classification} action that consists in choosing the final category of $x$. This action results in transiting from$z^{T_\theta(x)}(x)$ to $y_\theta(x)$ and ending the sequential process. At each step $C$ classification actions are available
\end{itemize}

A policy $\theta$ thus defines a probability of chosing an action knowing the state of the process. It has been demonstrated that the optimal policy in such a context is a deterministic policy which chooses at each step the best possible action. In the next parts, we first describe how a policy is parametrized through the set of parameters $\theta$ and how such a polciy provide a sparse classifier and allow us to avoid the selection of rares features.

\subsection{Parametrized Policy and Approximated Reinforcement Learning}

We consider here a scoring function $f_\theta$ which goal is to compute, for each possible state $s$ of the process and each possible action $a$, a score that refletcs how good it is to take action $a$ in state $s$ w.r.t to the reward function defined in the preivous part. This corresponds to the context of \textit{Approximated Reinforcement Learning} where one has to approximate a policy on a MDP throught the use of a function approximator instead of the tabular case often studied in reinforcement learning. This scoring function is defined as:
\begin{equation}
g:\begin{cases}
	\mathcal{X} \times \mathcal{Z} \times \mathcal{A} \rightarrow \mathbb{R} \\
	(x,z),a \rightarrow g_\theta( (x,z),a )
	\end{cases}
\end{equation}
where $x$ is the input to classify, $z$ is a subset of previously selected features and $a$ is an action in $\mathcal{A}$ as defined previously. $a$ can be euther a \textit{classification} action or a \textit{feature selection} action.



\subsubsection{Sparsity and OverFitting}


\subsection{Learning with Simulation}

\subsection{Complexity}


==> sections/taskdef.tex <==
\section{Task Definition and General Principles of the Approach}
 \label{sec:not-task}

	Let $\documents$ denote the set of all possible textual documents, and $\categories$ the set of $\nbcategories$ categories numbered from $1$ to $\nbcategories$. Each document $\doc{}$ in $\documents$ is associated with one or many\footnote{In this article, we consider both the mono-label classification task, where each document is associated to exactly one category, and the multi-label task where a document can be associated with many categories.} categories of $\mathcal{C}$. This label information is only known for a subset of documents $\documentstrain \subset \documents$ called training documents, composed of $\nbdocumentstrain$ documents denoted $\documentstrain=(\doc{1},...,\doc{\nbdocumentstrain})$. The labels of document $\doc{i}$ are given by a vector of scores $\scorecategorydocument{i}=(\scorecategorydocumentcategory{i}{1},...,\scorecategorydocumentcategory{i}{\nbcategories})$. We assume that:

\begin{equation}
		\scorecategorydocumentcategory{i}{k} = \begin{cases} 1 \text{ if } \doc{i} \text{ belongs to category } k \\
																												 0 \text{ otherwise}
																						\end{cases}.
\end{equation}
	
	 
	The goal of TC is to compute, for each document $d$ in $\documents$, the corresponding score for each category.  The classification function $f_\theta$ with parameters $\theta$ is thus defined as : 
	\begin{equation}
		f_\theta : \begin{cases} \documents : [0;1]^\nbcategories \\ d \rightarrow \scorecategorydocument{d} \end{cases}.
	\end{equation}
	Learning the classifier consists in finding an optimal parameterization $\theta^*$ that reduces the mean loss such that:
    \begin{align}\label{eq:min-theta}
        \theta^* = \argmin_{\theta} {1 \over N_{train}} \sum_{i=1}^{N_{train}} L(f_\theta(d_i), y^{d_i}),
    \end{align}
    where $L$ is a loss function proportional to the classification error of $f_\theta(d_i)$.
    
\vspace{-0.5cm}
\subsection{Overview of the approach}
\label{ioverview}
This section aims to provide an intuitive overview of our approach.  The ideas presented here are formally presented in Section \ref{sec:tc-sdp}, and will only be described in a cursory manner below.

\subsubsection{Inference} We propose to model the process of text classification as a sequential decision process.  In this process, our classifier reads a document sentence-by-sentence and can decide --- at each step of the reading process --- if the document belongs to one of the possible categories. 
This classifier can also chose to stop reading the document once it considers that the document has been correctly categorized. 

In the example described in Fig. \ref{fig:seqread}, the task is to classify a document composed of 4 sentences.  The documents starts off unclassified, and the classifier begins by reading the first sentence of the document. Because it considers that the first sentence does not contain enough information to reliably classify the document, the classifier decides to read the following sentence. Having now read the first two sentences, the classifier decides that it has enough information at hand to classify the document as \textit{cocoa}. 

The classifier now reads the third sentence and --- considering the information present in this sentence --- decides that the reading process is finished; the document is therefore classified in the \textit{cocoa} category.  

Had the document belonged to multiple classes, the classifier could have continued to assign other categories to the document as additional information was discovered.

\begin{figure}[h]
\begin{center}
\includegraphics[width=1.0\linewidth]{fig/ludo1.png}
\end{center}
\vspace{-0.5cm}
\caption{Inference on a document}
\label{fig:seqread}
\end{figure}

In this example, the model took four \textbf{actions}: \textit{next}, \textit{classify as cocoa}, \textit{next} and then \textit{stop}.  The choice of each action was entirely dependent on the corresponding \textbf{state} of the reading process. The choice of actions given the state, such as those picked while classifying the example document above, is called the \textbf{policy} of the classifier. 
This policy --- denoted $\pi$ --- consists of a mapping of states to actions relative to a score.  This score is called a Q-value --- denoted $Q(s,a)$ --- and reflects the worth of choosing action $a$ during state $s$ of the process. 
Using the Q-value, the inference process can be seen as a \textbf{greedy process} which, for each timestep, chooses the best action $a^*$ defined as the action with the highest score w.r.t. $Q(s,a)$:
\begin{equation}
a^*=\argmax\limits_{a} Q(s,a).
\end{equation}

\subsubsection{Training}The learning process consists in computing a $Q$-$function$\footnote{The \textit{Q-function} is an approximation of $Q(s,a)$} which minimizes the classification loss (as in equation \eqref{eq:min-theta}) of the documents in the training set. The learning procedure uses a monte-carlo approach to find a set of \textit{good} and \textit{bad} actions relative to each state.  \textit{Good} actions are actions that result in a small classification loss for a document. The \textit{good} and \textit{bad} actions are then learned by a statistical classifier, such as an SVM. 

An example of the training procedure on the same example document as above is illustrated in Fig \ref{fig:seqlearn}.  To begin with, a random state of the classification process is picked. Then, for each action possible in that state, the current policy is run until it stops and the final classification loss is computed. 
The training algorithm then builds a set of \textit{good} actions --- the actions for which the simulation obtains the minimum loss value --- and a set of remaining \textit{bad} actions. This is repeated on many different states and training documents until, at last, the model learns a classifier able to discriminate between \textit{good} and \textit{bad} actions relative to the current state. 

\begin{figure}[h]
\begin{center}
\includegraphics[width=0.8\linewidth]{fig/ludo2bis.png}
\end{center}
\vspace{-0.5cm}
\caption{Learning the sequential model. The different steps of one learning iteration are illustrated from left to right on a single training document.}
\label{fig:seqlearn}
\end{figure}

\vspace{-0.8cm}
\subsection{Preliminaries}

We have presented the principles of our approach and given an intuitive description of the inference and learning procedures.  We will now formalize this algorithm as a Markov Decision Process (MDP) for which an optimal policy is found via Reinforcement Learning. Note that we will only go over notations pertinent to our approach, and that this section lacks many MDP or Reinforcement Learning definitions that are not necessary for our explanation.

\subsubsection{Markov Decision Process}
	A Markov Decision Process (MDP) is a mathematical formalism to
model sequential decision processes.  We only consider deterministic MDPs, defined by a 4-tuple: $(\states,\actions,\transitions,\reward)$. Here, $\states$ is the set of possible states, $\actions$ is the is the set of possible actions, and $\transitions : S \times A
\rightarrow S$ is the state transition function such that $\transition{s}{a}\rightarrow s'$ (this symbolizes the system moving from state $s$ to state $s'$ by applying action $a$).  The reward, $\reward : S \times A \rightarrow \mathbb{R}$, is a value that reflects the quality of taking action $a$ in state $s$ relative to the agent's ultimate goal.  We will use $\possibleactions{s} \subseteq \actions$ to refer to the set of possible actions available to an agent in a particular state $s$.

An agent interacts with the MDP by starting off in a state $s \in \states$.  The agent then
chooses an action $a \in \possibleactions{s}$ which moves it to a new state $s'$ by applying the transition $\transition{s}{a}$. The agent obtains a reward $\rewardsa{s}{a}$ and then continues the process until it reaches a terminal state $s_{final}$ where the set of possible actions is empty i.e $\possibleactions{s_{final}}=\emptyset$. 

\subsubsection{Reinforcement Learning}
Let us define $\pi : S \rightarrow A$, a stochastic policy such that $\forall a \in A(s), \pi(s) = a$ with probability $P(a|s)$. The goal of RL is to find an optimal policy $\pi^*$ that maximizes the cumulative reward obtain by an agent. We consider here the finite-horizon context for which the cumulative reward corresponds to the sum of the reward obtained at each step by the system, following the policy $\pi$. The Reinforcement Learning goal is to  find the optimal policy denoted $\pi^*$  which maximizes the cumulative reward obtained for all the states of the process i.e:
\begin{equation}
\pi^* = \argmax_\pi \sum\limits_{s_0 \in \states} \mathbb{E}_{\pi}[\sum\limits_{t=0}^{T}r(s_t,a_t)]
\end{equation}

Many algorithms have been developed for finding such a policy, depending on the assumptions made on the structure of the MDP, the nature of the states (discrete or continuous), etc.  In many approaches, a policy $\pi$ is defined through the use of a $Q(s,a)$ which reflects how much reward one can expect by taking action $a$ on state $s$. With such a function, the policy $\pi$ is defined as:
\begin{equation}
\pi = \argmax\limits_{a \in \mathcal{A}(s)} Q(s,a)
\end{equation}
In such a case, the learning problem consists in finding the optimal value $Q^*$ which results in the optimal policy $\pi^*$.

Due to the very large number of states we are facing in our approach, we consider the Approximated Reinforcement Learning context where the $Q$ function is approximated by a parameterized function $Q_\theta(s,a)$, where $\theta$ is a set of parameters such as:
\begin{equation}
Q_\theta(s,a) = <\theta, \Phi(s,a)>
\end{equation}
where $<\cdot,\cdot>$ denotes the dot product, and $\Phi(s,a)$ is a feature vector representing the state-action pair $(s,a)$.  The learning problem consists in finding the optimal parameters $\theta^*$ that results in an optimal policy:
\begin{equation}
\pi^* = \argmax\limits_{a \in \mathcal{A}(s)} <\theta,\Phi(s,a)>.
\end{equation}


==> sections/tcsdp.tex <==
Formally, we consider that a document $\doc{}$ is composed of a sequence of sentences such that $\doc{}=(\sentence{\doc{}}{1},\hdots,\sentence{\doc{}}{\lengthdoc{\doc{}}})$, where $\sentence{\doc{}}{i}$ is the i-th sentence of the document and $\lengthdoc{\doc{}}$ is the total number of sentences making up the document.  Each sentence $\sentence{\doc{}}{i}$ has a corresponding feature vector --- a normalized tf-idf vector in our case --- that describes its content.

\vspace{-0.3cm}
\subsection{MDP for Multi-Label Text Classification}\label{sec:sdp-mdp}
 We can describe our sequential decision problem using an MDP.  Below, we describe the MDP for the multilabel classification problem, of which monolabel classification is just a specific instance:
\begin{itemize}
\item Each state $s$ is a triplet $(\doc{},p,\estimatedscorecategorydocumentcategory{})$ such that:
\begin{itemize}
\item $\doc{}$ is the document the agent is currently reading.
\item $p \in [1,\lengthdoc{\doc{}}]$ corresponds to the current sentence being read; this implies that $\sentence{\doc{}}{1}$ to $\sentence{\doc{}}{p-1}$ have already been read.
\item $\estimatedscorecategorydocumentcategory{}$ is the set of currently assigned categories --- categories previously assigned by the agent during the current reading process --- where $\estimatedscorecategorydocumentcategory{k} = 1$ iff the document has been assigned to category $k$ during the reading process, or $0$ otherwise.
\end{itemize}

\item The set of actions $\possibleactions{s}$ is composed of:
\begin{itemize}
\item One or many \textbf{classification} actions denoted \textit{classify as $k$} for each category $k$ where $\estimatedscorecategorydocumentcategory{k} = 0$.  These actions correspond to assigning document $\doc{}$ to category $k$.
\item A \textbf{next sentence} action denoted \textit{next} which corresponds to reading the next sentence of the document.
\item A \textbf{stop action} denoted \textit{stop} which corresponds to finishing the reading process.
\end{itemize}

\item The set of transitions $\transition{s}{a}$ act such that:
\begin{itemize}
\item $\transition{s}{classify as k}$ sets $\estimatedscorecategorydocumentcategory{k} \leftarrow 1$.
\item $\transition{s}{next}$ sets $p \leftarrow p+1$.
\item $\transition{s}{stop}$ halts the decision process.
\end{itemize}

\item The reward $\reward(s,a)$ is defined as:
\begin{align}
r(s,a) = \left\{
\begin{array}
{lll}
F_1(y,\hat{y})&\mbox{ if } a \textrm{ is a \textit{stop} action}\\
0&\mbox{otherwise}
\end{array}
\right .,
\end{align}
where $y$ is the real vector of categories for $d$ and $\hat{y}$ is the predicted vector of categories at the end of the classification process. The $F_1$ score of a single document is defined as:
\begin{align}
F_1(y,\hat{y}) &= 2 \cdot \frac{p(y,\hat{y}) \cdot r(y,\hat{y})}{p(y,\hat{y}) + r(y,\hat{y})}\\
&\text{ with }\\
 p(y,\hat{y}) = \sum\limits_{k=0}^C \mathds{1} (\hat{y_k} = y_k) / \sum\limits_{k=0}^C \hat{y_k} &\text{ and }r(y,\hat{y}) = \sum\limits_{k=0}^C \mathds{1} (\hat{y_k} = y_k) / \sum_{k=0}^C y_k
\end{align}
\end{itemize}

%
%A portion of the MDP for a three-class task is presented in figure \ref{fig:graph-multilabel}.
%\begin{figure}[h]
%%\includegraphics{fig/r8-train.png}
%\begin{center}
%%\includegraphics[width=.5\linewidth]{fig/graph-multi.pdf} \\
%\caption{A piece of the MDP for a three-class multilabel task.}
%\label{fig:graph-multilabel}
%\end{center}
%\end{figure}

\subsubsection{MDP for Mono-Label Text Classification}
In mono-label classification, we restrict the set of possible actions. The \textit{classify as k} action leads to a stopping state such that $A(s) = \{\textit{stop}\}$.  This way, once one label has been attributed the episode is over. Note that, in the case of a mono-label system --- where only one category can be assigned to a document --- the reward corresponds to a classical accuracy measure: $1$ if the chosen category is correct, and $0$ otherwise.


\vspace{-0.3cm}
\subsection{Features over states}
We must now define a feature function which provides a vector representation of a state-action pair $(s,a)$.  The purpose of this vector is to be able to present $(s,a)$ to a statistical classifier to know whether it is \textit{good} or \textit{bad}.  Comparing the scores of various $(s,a)$ pairs for a given state $s$ allows us to choose the best action for that state. 

Classical text classification methods only represent documents by a global --- and usually tf-idf weighted --- vector.  We choose, however, to include not only a global representation of the sentences read so far, but also a local component corresponding to the most recently read sentence. Moreover, while in state $s$, a document may have been already assigned to a set of categories; the feature vector $\Phi(s,a)$ must also include this information. The vector representation of a state $s$ is thus defined as $\Phi(s)$:
\begin{equation}
\Phi(s) = \left( \frac{ \sum\limits_{i=1}^{p} \sentence{\doc{}}{i} }{p} \text{          }  \sentence{\doc{}}{p} \text{          } \hat{y_0} \hdots  \hat{y_C} \right)
\end{equation}
$\Phi(s)$ is the concatenation of a set of sub-vectors describing: the mean of the feature vectors of the read sentences, the feature vector of the last sentence, the set of already assigned categories.

In order to include the action information, we use the block-vector trick introduced by \cite{Har-Peled2002} which consists in projecting $\Phi(s)$ into a higher dimensional space such that:
\begin{equation}
\Phi(s,a) = \left( 0 \hdots \phi(s) \hdots 0 \right),
\end{equation}
The position of $\Phi(s)$ inside the global vector $\Phi(s,a)$ is dependent on action $a$. This results in a very high dimensional space which is easier to classify in with a linear model.

% 
%\subsection{Reward function and Text Classification}
%As stated above, the goal of the agent is to find an optimal policy $\pi^*$ such that, for a starting state $s$ sampled from a distribution $D$:
%\begin{align} \label{eq:pol-def}
%\pi^*& = \argmax_\pi \mathbb{E}_{s \sim D}[R^\pi(s)].
%\end{align}
%Since there is only one a reward at the end of the episode, we can write the return as
%\begin{align} \label{eq:ret-rew}
%R^\pi(s) = r(\pi_{final}(s), \textit{stop}).
%\end{align}
%where $\pi_{final}(s)$ is the final state of an episode starting with state $s$, following policy $\pi$.
%
%We can rewrite \eqref{eq:pol-def} in a minimizing fashion
%\begin{equation}
%\pi^* = \argmin_\pi -{1 \over N} \overset{N}{\sum_{s \in D}}R^\pi(s), 
%\end{equation}
%and inject \eqref{eq:ret-rew} to obtain 
%\begin{equation}
%\pi^* = \argmin_\pi {1 \over N} \overset{N}{\sum_{s \in D}} {-F_1(\pi_{final}(s))}.
%\end{equation}
%If we consider $-1 \times F_1$ as the loss function of a statistical classifier, we show that searching for the optimal policy is equivalent to minimizing the loss of a classifier.
%\\
%XXX\\
%In the case of a monolabel classification problem, where $cat(\pi_{final}(s))$ is the predicted category, and $cat_{true}(s)$ is the real category.  This allows us to write
%\begin{align}
%F_1(s) = \left\{
%\begin{array}
%{lll}
%1&\mbox{ if } cat(\pi_{final}(s)) = cat_{final}(s)\\
%0&\mbox{ otherwise }
%\end{array}
%\right ..
%\end{align}
%Let us define a loss function for a predicted label $x$ and the correct label $y$:
%\begin{align}
%L(x,y) = \left\{
%\begin{array}
%{lll}
%0&\mbox{ if } x = y\\
%1&\mbox{ if } x \neq y
%\end{array}
%\right .,
%\end{align}
%
%which allows us to rewrite $(3)$ as
%
%\begin{align}
%\pi^* = \argmin_\pi {1 \over N} \sum L(\pi(s_{\mathbf{T}-1}), label(s))
%\end{align}
%Since $\pi(s_{\mathbf{T}-1})$ produces a labeling action, we can see that choosing the optimal policy based on $R^\pi$ is equivalent to the minimization of the loss function in \eqref{min_theta}.
%XXX
%\subsection{Learning with Rollouts}
%%%%Rollouts
%\label{sec:rollouts}
%An algorithm for implementing Approximate RL is Approximate Policy Iteration with Rollouts\cite{Lagoudakis2003}.  A set of states $D = \{s_1, \hdots, s_d\}$ is picked from the total state distribution as the learning set; $\tilde{R}_T^{\pi}(s,a) = R^\pi(T(s,a)) $ is estimated for each state-action pair:
%
%\begin{algorithm}\label{alg:rollout}
%\dontprintsemicolon
%\KwData{\\
%$\mathcal{M}$ : generative model\\
%$\pi_0$: initial policy\\
%$K$ : number of trajectories\\
%}
%\Repeat{$\pi\sim\pi'$}{
%$\pi = \pi'$\\
%$\mathbf{TS}=\emptyset$\\
% \ForEach{$s \in D$}{
%  \ForEach{$a \in A$}{
%   $\tilde{R}_T^{\pi}(s,a) \leftarrow \mathbf{Rollout}(\mathcal{M},s,a,K)$\\
%  }
%  $a^* = argmax_{a \in A} \tilde{R}_T^{\pi}(s,a)$\\
%  \If{$\forall a \in A, a \neq a^* : \tilde{R}_T^{\pi}(s,a) \tilde{<} \tilde{R}_T^{\pi}(s,a)$}{
%   $\mathbf{TS} \leftarrow \mathbf{TS} \bigcup \{(s,a)^+\}$\\
%  }
%  \ForEach{$\forall a \in A, a \neq a^* : \tilde{R}_T^{\pi}(s,a) \tilde{<} \tilde{R}_T^{\pi}(s,a)$}{
%  $\mathbf{TS} \leftarrow \mathbf{TS} \bigcup \{(s,a)^-\}$\\
%  }
%  $\pi' = \mathbf{Learn}(\mathbf{TS})$
% }
%}
%\Return{ $\pi$}
%\caption{API with Rollouts for Return Value}
%\end{algorithm}
%
%    Once a good number of states have been visited, and the best action (the action giving the highest return) is calculated for each state, the set of state-action pairs is split into two parts: pairs that include the best action for that state (labelled as $\{s,a\}^+$), and the remaining pairs ($\{s,a\}^-$).  
%A classifier is then trained on these two sets to predict whether a state-action pair includes the best action
%or not.  The parametric aspect of the classifier allows us to remember the state-action
%pairs visited without consuming much memory.  The generalizing
%capacities of the classifier allow us to give estimates of best
%state-action pairs even if we have never visited them.  Unfortunately, the
%classifier will not be able to learn perfectly
%and is therefore only providing an estimate of $\pi$.%, which we will call $\hat{\pi}$.
%
%The $\mathbf{Rollout(\mathcal{M}, s, a, K)}$ function used in Algorithm \ref{alg:rollout} estimates $R_T^\pi(s,a)$ by taking a state-action pair $(s,a)$ and running a policy $\pi$ starting at $T(s,a)$ until the end of the episode.  This is done $K$ times to get a better estimation of $R_T^\pi(s,a)$ since our policy is stochastic.
\vspace{-0.3cm}
\subsection{Learning and Finding the optimal classification policy}

In order to find the best classification policy, we used a recent Reinforcement Learning algorithm called \textit{Approximate Policy Iteration with Rollouts}. In brief, this method uses a monte-carlo approach to evaluate the quality of all the possible actions amongst some random sampled states, and then learns a classifier whose goal is to discriminate between the \textit{good} and \textit{bad} actions relative to each state. Due to a lack of space, we do not detail the learning procedure here and refer to the paper by Lagoudakis et al \cite{Lagoudakis2003}. An intuitive description of the procedure is given in Section \ref{ioverview}.


